Joint Pricing and Rebalancing of Autonomous Mobility-on-Demand Systems

This paper studies optimal pricing and rebalancing policies for Autonomous Mobility-on-Demand (AMoD) systems. We take a macroscopic planning perspective to tackle a profit maximization problem while ensuring that the system is load-balanced. We begin by describing the system using a dynamic fluid model to show the existence and stability of an equilibrium (i.e., load balance) through pricing policies. We then develop an optimization framework that allows us to find optimal policies in terms of pricing and rebalancing. We first maximize profit by only using pricing policies, then incorporate rebalancing, and finally we consider whether the solution is found sequentially or jointly. We apply each approach on a data-driven case study using real taxi data from New York City. Depending on which benchmarking solution we use, the joint problem (i.e., pricing and rebalancing) increases profits by 7% to 40%

==> sections/Stability-equilibrium-sets.tex <==
\subsection{Stability of equilibrium sets}
\SW{we can include the exact same analysis as in \cite{Pavone2012}}
Let $\bu \in \scrU$ and $m>m_\bu$. Then, an equilibrium exists. Now let us define the following
\begin{definition}
    Let a set of solutions $\scrE_\bu$ be \emph{locally asymptotically stable} if for any equilibrium $(\bc',\bv')\in\scrE_\bu$ there exists a neighborhood $\scrB_\bu^\delta(\bc',\bv')$ such that the evolution of the model starting at:
    \begin{align*}
        c_i(t)=c_i', \text{ for } \tau \in [ - \max T_{ij},0 ) \\
        v_i(t)=v_i', \text{ for } \tau \in [ - \max T_{ij},0 ) \\
        (\bc(0), \bv(0)) \in \scrB^\delta_\bu(\bc', \bv') 
    \end{align*}
    has a limit which belongs to the equilibrium set. In other words $(\lim\limits_{t \xrightarrow{} \infty}\bc(t), \lim\limits_{t \xrightarrow{} \infty}\bv(t)) \in \scrE_\bu$. Where:
   \begin{align*}
        & \scrE_\bu :=  \{(\bc, \bv)|c_i=0, v_i>0 \quad \forall i \in \scrN, \quad \sum\limits_i v_i=m-m_\bu  \} \\
        & \scrB^\delta_\bu :=  \{ (\bc, \bv)|c_i \geq 0, v_i>0 \quad \forall i \in \scrN, \quad ||\bc-\bc', \bv-\bv'|| \leq \delta,  \quad \sum\limits_i v_i=m-m_\bu   \}
    \end{align*} 
    
\begin{theorem}
    Let $\bu \in \scrU$ be a feasible price vector and assume $m>m_\bu$. Then, the set of equilibria $\scrE_\bu$ is locally asymptotically stable. 
\end{theorem}

\begin{proof}
    follows the same analysis as in \cite{Pavone2012}, see appendix.
\end{proof}
\end{definition}
